Virtual Category Learning: A Semi-Supervised Learning Method for Dense Prediction with Extremely Limited Labels

Due to the costliness of labelled data in real-world applications, semi-supervised learning, underpinned by pseudo labelling, is an appealing solution. However, handling confusing samples is nontrivial: discarding valuable confusing samples would compromise the model generalisation while using them for training would exacerbate the issue of confirmation bias caused by the resulting inevitable mislabelling. To solve this problem, this paper proposes to use confusing samples proactively without label correction. Specifically, a Virtual Category (VC) is assigned to each confusing sample in such a way that it can safely contribute to the model optimisation even without a concrete label. This provides an upper bound for inter-class information sharing capacity, which eventually leads to a better embedding space. Extensive experiments on two mainstream dense prediction tasks -- semantic segmentation and object detection, demonstrate that the proposed VC learning significantly surpasses the state-of-the-art, especially when only very few labels are available. Our intriguing findings highlight the usage of VC learning in dense vision tasks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/6_differences.tex <==

\onecolumn

\setcounter{section}{0}
\def\thesection{\alph{section}}

\section{Summary of Differences}

This paper substantially extends our preliminary study presented in ECCV oral \cite{chen2022semisupervised}. The major novelties and differences are described as follows:

\begin{itemize}
\item We extend VC learning to semi-supervised semantic segmentation to evaluate its generalisation ability on dense vision tasks. Extensive experiments demonstrated that a straightforward semi-supervised semantic segmentor with VC learning exceeds state-of-the-art methods by a large margin.

\item We explored two effective methods for the potential category set creation based on the specificity of semantic segmentation. They can also serve as a confusing sample discovery algorithm to facilitate many semi-supervised solutions, such as the pseudo label correction.

\item We also propose a new module to generate the virtual weight in VC learning. 
\item The paper is re-organised for a better presentation. Specifically, in~\cref{sec:related}, we introduced the progress and problems of semi-supervised learning on semantic segmentation and object detection. \cref{sec:method}~abstracts our method for dense vision tasks as a general one-pixel classification to illustrate the proposed algorithm more clearly. We also provide the pseudo-code and the hyperparameters in~\cref{sec:exp}. The mathematical derivation without the smooth approximation we used in our ECCV paper is provided in~\cref{subsec:math}, demonstrating the feasibility of VC learning in several aspects.

\item More experiments and ablation studies with detailed analyses are conducted.
\begin{itemize}
    \item{\textbf{Experiments}}
    \begin{itemize}
        \item{\cref{tab:seg-voc}: semantic segmentation performance on Pascal VOC.}
        \item{\cref{tab:seg-city}: semantic segmentation performance on Cityscapes.}
        \item{\cref{tab:seg-backbone}: semantic segmentation performance on Pascal VOC with different backbones.}
        \item{\cref{tab:acc-cls-res18}: classification performance on miniImageNet.}
    \end{itemize}

    \item{\textbf{Ablation Studies}}
    \begin{itemize}
        \item{\cref{fig:baseline-seg}: the mIoU of the teacher-student baseline segmentor reveals its problem.}
        \item{\cref{fig:ablation-seg-a}: the ablation study of the policies for confusing samples.}
        \item{\cref{fig:ablation-seg-b}: the ablation study of the potential category set creation methods and the virtual weight generation module.}
        \item{\cref{fig:ablation-seg-c}: the trend of confusing samples ratio.}
        \item{\cref{fig:ablation-seg-d}: the accuracy of pseudo labels.}
        \item{\cref{tab:seg-mse-loss}: the ablation study of different loss forms.}
        \item{\cref{fig:ablation-seg-vc-area} and \cref{fig:ablation-det-pc-vis}: the visualisation of potential category sets.}
        \item{\cref{fig:ablation-seg-results}: the qualitative results.}
        \item{\cref{sec:det-ablation}: some additional ablation studies for detection.}
    \end{itemize}
\end{itemize}

\end{itemize}
